Explaining Relationships Between Scientific Documents

We address the task of explaining relationships between two scientific documents using natural language text. This task requires modeling the complex content of long technical documents, deducing a relationship between these documents, and expressing the details of that relationship in text. In addition to the theoretical interest of this task, successful solutions can help improve researcher efficiency in search and review. In this paper we establish a dataset of 622K examples from 154K documents. We pretrain a large language model to serve as the foundation for autoregressive approaches to the task. We explore the impact of taking different views on the two documents, including the use of dense representations extracted with scientific IE systems. We provide extensive automatic and human evaluations which show the promise of such models, but make clear challenges for future work.

==> eval_dontuse.tex <==
\section{Evaluation}
\label{sec:eval}

\subsection{Baseline}
While neural text generation techniques have advanced significantly in recent years, their outputs are still inferior to human authored texts.
For some tasks, it is better to retrieve a relevant human-authored text than to generate novel text automatically \citep{Fan2018HierarchicalNS}. 
To test this, we use an information retieval baseline. 
Given a test instance input $(S,C)$ for principal $S$ and cited document $C$, we find the set $\mathbf{N}_C$, the nearest neighbors to $C$ in the training data.
For each document $N_C$ from  $\mathbf{N}_C$, let $\mathbf{N}_S$ be the set of documents that cite $N_C$.
This means that each $N_S \in {\mathbf N}_S$ contains at least one \citingsent $t'$ which cites $N_C$. 
We return the $t'$ associated with the $(N_S,N_C)$ pair from the training which is closest to $(S,C)$.

We measure the closeness of two pairs of documents by measuring cosine distances between vector representations of their abstracts.
The abstract of each document is encoded as a single dense vector by averaging the contextualized embeddings provided by the SciBERT model of \citet{Beltagy2019SciBERT} and normalizing.
%\footnote{Unlike the special version of SciGPT used in this work, we cannot guarantee that the pretrained SciBERT has not been exposed to documents from the training data.}
The distance between $(S,C)$ and candidate $(N_S,N_C)$ is computed as:
\begin{equation}
    \alpha\cos(S,N_S)+\beta\cos(C,N_C)
\end{equation}
where $\alpha$ and $\beta$ control the relative contribution of the two document similarities. 
We explore setting both $\alpha$ and $\beta$ to 1, or tuning them to optimize BLEU on the validation data.

\subsection{Automatic Evaluation}


\begin{table*}[t]
    \centering
    \begin{tabular}{rlrrr}
        \toprule
         && {\bf BLEU} & {\bf ACL-BLEU} & {\bf Rouge-L} \\ \toprule
        \multirow{3}{*}{\textsc{SciGen}} & \source~abs $\times$ cited abs &9.82 &10.40 & 8.4   \\
        %&abs $\times$ intro &9.39 & 9.82 &  8.4 \\
        %&abs $\times$ sample &9.60 &10.48 &  8.5 \\ \cline{2-5}
        &\source~intro $\times$ cited abs &9.92 &11.22 &      8.7 \\
        %&intro $\times$ intro &9.80 &10.54 &    8.8  \\
        %&intro $\times$ sample & 9.81 & 10.31 &     8.7 \\
        \midrule \midrule
        %\cline{2-7}
        \multirow{2}{*}{IR} & \source~abs $\times$ cited abs& 9.93 & 10.50  &    9.7 \\
        & \hspace{1em} + MERT (BLEU)& 10.23 & 10.29  &   9.8 \\
        %& no \source~$\times$ abs & 9.79 &-  &     9.6 \\
        \bottomrule
    \end{tabular}
    \caption{Automatic evaluation of generated texts. Though we evaluated all variants, above only shows the best performing models of each class (see Appendix for all results). The ACL-BLEU column denotes the BLEU scores of the subset of examples we use for human evaluation. Statistical significance is discussed in Section~\ref{sec:eval}.}
    \label{tab:autometrics}
\end{table*}
\begin{table*}
\centering
\begin{tabular}{lllcccc}
\hline
&
\fieldheading{Method} & \fieldheading{Context}& \fieldheading{BLEU} & \fieldheading{Rouge-1} & \fieldheading{Rouge-2} & \fieldheading{Rouge-L}\\
\hline
\multirow{4}{*}{\shortstack{\citeauthor{luu2020citation}\\\citeyearpar{luu2020citation}}} & \multirow{2}{*}{generation} & source abs $\times$ cited abs &  9.82 & 0.107 & 0.006 & 0.084\\
& & source intro $\times$ cited abs &  9.92 & 0.111 & 0.010 & 0.087\\
\cline{2-7}
& \multirow{3}{*}{retrieval } & source abs $\times$ cited abs & 9.93 & 0.142 & 0.007 & 0.097\\
& & $\quad$+MERT & 10.23 & 0.143 & 0.007 & 0.098\\
& & no source $\times$ cited abs & 9.79 & 0.141 & 0.006 & 0.096\\
\hline
\multirow{8}{*}{This work} & \multirow{4}{*}{generation} & source abs $\times$ cited tfidf & 11.82 & 0.148 & 0.008 & 0.115\\
& & source intro $\times$ cited tfidf & 13.17 & 0.150 & 0.013 & 0.120\\
& & source abs $\times$ cited entities & 13.10 & 0.143 & 0.008 & 0.114\\
& & source intro $\times$ cited entities & 13.41 & 0.147 & 0.014 & 0.118\\
\cline{2-7}
& \multirow{4}{*}{\shortstack{generation \\and \\ranking}} & source abs $\times$ cited tfidf & 11.61 & 0.150 & 0.009 & 0.115\\
& & source intro $\times$ cited tfidf & 13.50 & 0.155 & 0.016 & 0.123\\
& & source abs $\times$ cited entities & 13.28 & 0.147 & 0.010 & 0.116\\
& & source intro $\times$ cited entities & 13.16 & 0.150 & 0.013 & 0.118\\
\hline
\multirow{8}{*}{\shortstack{This work \\ (rerun rouge \\ w/ pyrouge)}} & \multirow{4}{*}{generation} & source abs $\times$ cited tfidf & 11.82 & 0.182 & 0.013 & 0.127\\
& & source intro $\times$ cited tfidf & 13.17 & 0.186 & 0.020 & 0.135\\
& & source abs $\times$ cited entities & 13.10 & 0.186 & 0.015 & 0.133\\
& & source intro $\times$ cited entities & 13.41 & 0.189 & 0.019 & 0.134\\
\cline{2-7}
& \multirow{4}{*}{\shortstack{generation \\and \\ranking}} & source abs $\times$ cited tfidf & 11.61 & 0.189 & 0.015 & 0.130\\
& & source intro $\times$ cited tfidf & 13.50 & 0.193 & 0.021 & 0.139\\
& & source abs $\times$ cited entities & 13.28 & 0.191 & 0.016 & 0.135\\
& & source intro $\times$ cited entities & 13.16 & 0.194 & 0.019 & 0.136\\
\hline
\end{tabular}
\caption{\label{table:auto_eval} Automatic Evaluation.}
\end{table*}


\begin{table*}[t]
    \centering
    \begin{tabular}{lccc|c}
        % \toprule
        %  & {\bf Plausible} & {\bf Specific} & {\bf Correct} & {\it agreement}\\\hline
        % IR & 48.7 & 71.1&  38.9 & {\it 68.0}\\
        % {\sc SciGen} & 72.7 & 67.8 & 56.0 & {\it 61.8}\\
        % Gold & 76.9 & 82.4 &  65.0 & {\it 79.0 }\\\hline
        % {\it agreement }& {\it 71.0} & {\it 65.9} & {\it 66.0 }\\
        % \bottomrule 
        \toprule
         & {\bf Plausible} & {\bf Specific} & {\bf Correct} & {\it agreement}\\\hline
        IR (abs $\times$ abs) & 68.2 & 74.8 &  46.3 & {\it 77.5}\\
        {\sc SciGen} (intro $\times$ abs) & 87.5 & 72.3 & 64.0 & {\it 70.5}\\
        Gold & 89.0 & 81.4 &  72.1 & {\it 83.8 }\\\hline
        {\it agreement }& {\it 87.4} & {\it 69.8} & {\it 71.4 }\\
        \bottomrule 
    \end{tabular}
    \caption{Human evaluation of {\sc SciGen} and IR systems compared with gold \citingsent (percentages).}
    \label{tab:human1}
\end{table*}

We compare the different baseline systems using BLEU \citep{papineni2002bleu} and ROUGE  (specifically L; \citealp{Lin2004ROUGEAP}).
%, and the recently introduced BertScore \citep{Zhang2019BERTScoreET}, a similarity metric based on BERT embeddings which has been shown to correlate well with human judgments on other tasks. 
%To adapt the BertScore metric to the scientific text domain, we use SciBERT embeddings. 
Table~\ref{tab:autometrics} (above the double line) shows the performance of the {\sc SciGen} model on the test set when provided with the different input context combinations outlined in Section~\ref{sec:ntg}.
We find that context does make a difference for this category of model, and that a slight performance improvement comes from using the introduction of the \source~document rather than the abstract. 
Automatic evaluation of the retrieval-based methods on the test data is shown below the double line in Table~\ref{tab:autometrics}. 
We see that tuning the $\alpha$ and $\beta$ parameters to optimize BLEU on the validation set does lead to improved performance at test time, but the effect is less pronounced under other metrics. 
We also evaluate a model which uses only the cited document to retrieve \citingsents, ignoring the \source. 
This model does surprisingly well, indicating the importance of modeling the cited document in this task. 
We discuss this in more detail in Section~\ref{sec:analysis}.
%However, the human evaluation described below complicates this picture.
%We also observe that tuning the $\alpha$ and $\beta$ parameters on the validation set results in overfitting for this method. 
%Outputs are largely unchanged by this tuning; fewer than 400 test datapoints differ from the untuned outputs.
%A larger validation split may alleviate this problem. 

We assess statistical significance for select results using bootstrapping with 1000 samples in each of 100 iterations. 
This test shows that conditioning on the introduction of the \source~document improves performance compared to conditioning on the abstract when using the {\sc SciGen} model. 
However, we see that IR methods perform better than the best neural models under these metrics.\footnote{$p<0.01$ after Bonferonni correction for both cases.} We do not find enough evidence to reject the null hypothesis that any particular representation of the cited document's content (abstract, intro, or random sample) is preferable to the others. 

%\kelvin{ we need to qualify this better maybe: under the ACL subset, scigen is better}


% \begin{table*}[t]
%     \centering
%     \begin{tabular}{lllcc|cc}
%         \toprule
%         &&& \multicolumn{2}{c}{{\sc SciGen} (abs $\times$ abs)} & \multicolumn{2}{c}{IR (untuned)} \\
%     \toprule
%          & &&{\bf One Visible} & {\bf Both Visible}  & {\bf One Visible} & {\bf Both Visible} \\\hline
%      \multirow{3}{3pt}{\rotatebox[origin=c]{90}{\parbox{1.2cm}{\bf Source}}} && Believable & 32 & 22 & 37 & 23\\
%       & &Content-Dependent &12& 8  & 5 & 1\\
%       & &Not Believable & 6 & 20 & 8 &26 \\
       
%         \midrule
%      \multirow{3}{3pt}{\rotatebox[origin=c]{90}{\parbox{0.8cm}{\bf Cited}}} && Believable & 24  & 19 & 17 & 16\\
%       & &Content-Dependent & 8& 6  & 2 & 0\\
%       & &Not Believable & 18 & 25 & 31 & 34 \\
       
       
%         \bottomrule
%     \end{tabular}
%     \caption{Error analysis of {\sc SciGen} and {\sc IR}  generated texts.}
%     \label{tab:erroranalysis}
% \end{table*}

\subsection{Human Evaluation}

\kelvin{I'm debating between re-adding the table here or inline examples.}

We conduct a human evaluation of the generated text to determine how {\it correct}, {\it specific}, and {\it plausible} these outputs are given a particular pair of \source~ and cited abstracts.
By correct we mean: does the generated sentence correctly express the factual relationship between the \source~and cited documents?
We are also interested in specificity, as generic statements such as ``[The principal document] extend[s] the ideas of Chomsky and Halle (1968)'' \kelvin{can we do this? slightly modify it to better portray it? or is that just lying at that point? }, which may be factual, do not express a detailed understanding of the documents' relationship. 
We ask judges whether the generated sentence describes a specific relationship between the two works or is vague enough to be used to cite many different papers. 
A \citingsent can be specific even it is incorrect. 
Lastly, we define a \textit{plausible} \citingsent as one which could believably fit into the \source~document. 
Plausibility judgments give us a measure of how well \source~topicality and tone is captured without penalizing factual errors about the cited document. 

To measure plausibility, we show judges a \source~abstract and \citingsent; for specificity and correctness, judges are shown \source~and cited documents' abstracts along with a \citingsent. 
To ensure no annotator sees the output of more than one system on each datapoint, we randomly select 50 datapoints for each system from the subset of our test data whose \source~documents appear in the ACL anthology. 
We collect judgments from 37 NLP researchers with varying levels of expertise, the majority of whom are graduate students. 
Each judge is given 15 datapoints for each of the plausibility, specificity, and correctness qualities.
Judges are shown a table of datapoints asked to mark whether each meets ("Yes") or fails to meet ("No") the condition. 
Judges are permitted to label "?" or skip examples they feel uncertain about or unqualified to judge, which we ignore.

We compare the {\it \source~intro $\times$ cited abs} {\sc SciGen} setting against the untuned IR system. 
For calibration, we also elicit judgments for the gold \citingsent, which were citing sentences, extracted from \source~documents along with the correct \source~and cited abstracts. 
In total we collect over 1200 judgments, with over 100 for each system/quality combination. 
Since the distribution of this subset we assign for human evaluation differs from the overall test set, we also report BLEU on this subset in Table~\ref{tab:autometrics}. Notably, the SciGen systems perform as well or better than IR systems in this set. This change in performance may hint at differences in how different sub-fields in computer science cite prior work, though study is required to qualify these differences. 

Table~\ref{tab:human1} shows the percentage of ``yes'' judgments versus the total of ``yes'' and ``no'' judgements for each system/quality combination, along with pairwise agreement rates.
That gold texts do not achieve perfect scores demonstrates a limitation of our evaluation setup, due in part to the fact that judgments are based on document abstracts rather than their full texts. 
Still, we observe the highest scores for all text qualities over the gold text, as well as the highest agreement rate. 
%We can also see that, despite the IR system's strong performance in automatic metrics, it produces implausible and incorrect citing sentences more often than not.
We can also see that IR systems tend to produce implausible and incorrect \citingsent more often than not. A more sophisticated IR system could perhaps achieve better results.
The {\sc SciGen} system performs quite well in this analysis, with a majority of outputs deemed correct and plausibility ratings approaching those of the gold texts. 
We observe a larger difference in terms of specificity between {\sc SciGen} and gold texts, indicating that {\sc SciGen}, like many neural text generation systems, often generates vague and generic sentences. These generations tended to be vacuous such as ``\textsc{(Cited)} This work is an extension of the paper.'' Specificity is key for future downstream applications such as automated literature review and will need to be improved for those tasks.

\paragraph{Correlation with Automatic Metrics} 
To determine if any of the studied automatic metrics correlate with any of the human evaluated text qualities, we conduct a correlation analysis.
Specifically, for Rouge-L and BLEU we compare the distribution of scores between the outputs of automatic systems and their human judgments of plausibility, specificity, and correctness.
For outputs which have been assessed by multiple judges, we include the metric score for that output in the corresponding distribution once per judgment. 

To compare the continuous scores of the automatic metrics with categorical human judgements (which are dichotomous nominal variables), we compute a variant of Pearson correlation called point biserial correlation \cite{lev1949point}.
We find no significant correlation between any judged text quality and automatic metrics for the IR system. 
However, we do find a weak correlation between the BLEU scores of {\sc SciGen} and their human evaluation scores for correctness ($r_{pb} = 0.29, p < 0.01$ after Bonferroni correction). 
A box plot of the {\sc SciGen} BLEU scores by correctness category is presented in Figure~\ref{fig:box}.
We can see a difference in the means of these distributions, but the variance of incorrect responses is great.
Extended human evaluations on correctness may improve the sharpness of this contrast. 
Further, introducing a domain-specific term weighting to the BLEU metric may increase its ability to act as an approximation to correctness in future model development. 
These are promising directions for future work. 

\begin{figure}
    \centering
    \includegraphics[width=0.46\textwidth]{correctnes_boxplot.png}
    \caption{Box plot of BLEU scores by correctness judgment category for {\sc SciGen} system. }
    \label{fig:box}
\end{figure}
\begin{table*}[t]
    \centering
    \begin{tabular}{lcc|c}
        % \toprule
        %  & {\bf Plausible} & {\bf Specific} & {\bf Correct} & {\it agreement}\\\hline
        % IR & 48.7 & 71.1&  38.9 & {\it 68.0}\\
        % {\sc SciGen} & 72.7 & 67.8 & 56.0 & {\it 61.8}\\
        % Gold & 76.9 & 82.4 &  65.0 & {\it 79.0 }\\\hline
        % {\it agreement }& {\it 71.0} & {\it 65.9} & {\it 66.0 }\\
        % \bottomrule 
        \toprule
         & {\bf Specific} & {\bf Correct} & {\it agreement}\\\hline
        {\sc SciGen} (intro $\times$ abs) & 72.3 & 64.0 & {\it 70.5}\\
        IR (abs $\times$ abs) & 74.8 &  46.3 & {\it 77.5}\\
        Gold & 81.4 &  72.1 & {\it 83.8 }\\\hline
        {\it agreement }& {\it 69.8} & {\it 71.4 }\\
        \bottomrule 
    \end{tabular}
    \caption{ Human evaluation of {\sc SciGen} and IR systems compared with gold \citingsents{} (percentages).}
    \label{tab:human1}
\end{table*}

==> fact.tex <==

\section{Entity-Based Ranking}
\label{sec:fact}
\citet{maynez2020faithfulness} points out that extrinsic hallucinations happen frequently in summarization systems.
The ranking mechanism is aim at reducing such hallucinations by rewarding generated sentences with higher coverage of important entities.

We use the generation system in Section \ref{sec:terms} to independently generate $k$ citation sentences for each pair of $\langle S', C\rangle$. 
Those sentences are denoted as $\hat{t}^{(1)}, \hat{t}^{(2)},...,\hat{t}^{(K)}$.
For each $\hat{t}^{(k)}$, $1\leq k\leq K$, we again use DyGIE++ \citep{Wadden2019EntityRA} to extract entities $q_1^{(k)},q_2^{(k)},...,q_{Q^(k)}^{(k)}$.
We then calculate the mean reciprocal rank (MRR) for each of the $k$ sentences
\begin{equation}
    MRR = \frac{1}{Q^{(k)}}\sum_{\alpha=1}^{Q^{(k)}}\frac{1}{rank_{\alpha}^{(k)}}
\end{equation}
where $rank_{\alpha}^{(k)}$ is the rank of $q_{\alpha}^{(k)}$ in the sorted entity list $e_1,e_2,...,e_E$ from cited articles. $q_{\alpha}^{(k)}$ and $e_{j}$ is considered a match if their similarity score calculated by difflib is greater than or equal to $0.7$. In that case, $rank_{\alpha}^{(k)} = j$. If a $q_{\alpha}^{(k)}$ does not have a match, then $rank_{\alpha}^{(k)} = \infty$ and consequently, $\frac{1}{rank_{\alpha}^{(k)}} = 0$.

\subsection{Manual Analysis}
We conducted a manual correctness analysis of the generated texts. 
Two of the authors judged 50 datapoints from each system. 
They made use of the full text of both the principal and cited document to determine correctness. 
Correctness was judged on a 3-way scale: Correct; Too Vague (but not incorrect); and Incorrect. 
After judging all datapoints independently, the two authors discussed disagreements until a consensus was reached. 

The results of this analysis are shown in Table~\ref{tab:human2}.
We see a slight increase in correctness with the reranked TF-IDF model compared to the Intro $\times$ Abs model, though the difference here is smaller than the difference in BLEU scores between these two systems. c

\begin{table}[t]
    \centering
    \begin{tabular}{l|ccc}
    & Correct & Vague & Incorrect \\ \hline
    Intro $\times$ Abs & 11 & 7 & 32 \\
    Reranked TF-IDF & 13 & 6 & 31 
    \end{tabular}
    \caption{Results of Manual Analysis }
    \label{tab:human2}
\end{table}

==> model2.tex <==


\section{Citation Generation with Condensed Context}\label{sec:model_generation}

\xinyi{Notations are slightly different from Kelvin's paper}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/diagram.png}
    \caption{Diagram.}
    \label{fig:diagram}
\end{figure}


Given that $S\backslash t$ and $C$ are usually long, we select part of their tokens as the context provided to the model, denoted as $S'$ and $C'$ respectively. 
Therefore, instead of using Equation \ref{eq:prob}, we approximate that with
\begin{equation}
    P(t\mid S',C')
    \label{eq:prob}
\end{equation}

In the setting of a GPT-2 model, the probability of each token $t_{i}$ in $t$ is calculated in an auto-regressive manner:
\begin{equation}
\begin{aligned}
P(t_{i}\mid S',C',t_1,\ldots,t_{i-1}) = \\\textrm{GPT2}(S',\mho_{s\_c},C',\mho_{c\_t},t_1,\ldots,t_{i-1} \mid \theta)
\label{eq:gpt}
\end{aligned}
\end{equation}
where $\mho_{s\_c}$ and $\mho_{c\_t}$ are special tokens to separate $S'$ from $C'$, and $C' $ from $t$.

\citet{luu2020citation} chose $S'$ to be abstract or introduction, and chose $C'$ to be abstract, introduction or sampling. 
We follow their choices of $S'$, but experiment to use tf-idf or entities for $C'$.

\paragraph{Tf-idf} 
Tf-idf is short for term frequency–inverse document frequency. It is a measure of the frequency of a term in a document, normalized by the frequency of that token in all documents. In our case, we use unigrams as terms. We calculate the tf-idf score for each term in each document. Then, we keep the 100 terms with highest tf-idf scores for each document, and sort them in a descending order of scores. A special token $\mho_{tfidf}$ is then put between terms. The purpose of that special token is to distinguish the list of terms from a natural language sentence.
The resulting $C'$ is $w_1 ~\mho_{tfidf} ~w_2 ~\mho_{tfidf} ~...~\mho_{tfidf}~w_{100}$, where $w_i$ is the unigram with $i$-th ($1\leq i\leq 100$) highest tf-idf score.

\paragraph{Entities}
We extract entities from abstract using DyGIE++ \citep{Wadden2019EntityRA} trained on SciERC \citep{luan2018multi}.
DyGIE++ is an information extraction framework that enumerates, refines and scores text spans.
It is designed to capture both within-sentence and cross-sentence context.
We choose the model trained on SciERC \citep{luan2018multi} because SciERC, as a dataset for scientific articles, is the closest to our dataset.
After the entities are extracted, they are then sorted by tf-idf scores. Similar as above, a special token $\mho_{entity}$ is put between entities.
Given that only entities in abstracts are included here, we append tfidf tokens extracted from entire cited article to the end of the entities, until the window is full. 
In that case, $C'$ is considered as $e_1 ~\mho_{entity} ~e_2 ~\mho_{entity} ~... ~\mho_{entity} ~e_{E} ~\mho_{tfidf} ~w_1 ~...$, where $e_j$ ($1\leq j\leq E$, $E$ is the number of unique entities in abstract) is the entity with the $j$-th highest tf-idf score.

\subsection{Entity-Based Ranking}\label{subsec:model_ranking}
\citet{maynez2020faithfulness} points out that extrinsic hallucinations happen frequently in summarization systems.
The ranking mechanism is aim at reducing such hallucinations by rewarding generated sentences with higher coverage of important entities.

We use the generation system in Section \ref{subsec:model_generation} to independently generate $k$ citation sentences for each pair of $\langle S', C\rangle$. 
Those sentences are denoted as $\hat{t}^{(1)}, \hat{t}^{(2)},...,\hat{t}^{(K)}$.
For each $\hat{t}^{(k)}$, $1\leq k\leq K$, we again use DyGIE++ \citep{Wadden2019EntityRA} to extract entities $q_1^{(k)},q_2^{(k)},...,q_{Q^(k)}^{(k)}$.
We then calculate the mean reciprocal rank (MRR) for each of the $k$ sentences
\begin{equation}
    MRR = \frac{1}{Q^{(k)}}\sum_{\alpha=1}^{Q^{(k)}}\frac{1}{rank_{\alpha}^{(k)}}
\end{equation}
where $rank_{\alpha}^{(k)}$ is the rank of $q_{\alpha}^{(k)}$ in the sorted entity list $e_1,e_2,...,e_E$ from cited articles. $q_{\alpha}^{(k)}$ and $e_{j}$ is considered a match if their similarity score calculated by difflib is greater than or equal to $0.7$. In that case, $rank_{\alpha}^{(k)} = j$. If a $q_{\alpha}^{(k)}$ does not have a match, then $rank_{\alpha}^{(k)} = \infty$ and consequently, $\frac{1}{rank_{\alpha}^{(k)}} = 0$.

